Realizing Lattice Surgery on Two Distance-Three Repetition Codes with Superconducting Qubits

Quantum error correction is needed for quantum computers to be capable of fault-tolerantly executing algorithms using hundreds of logical qubits. Recent experiments have demonstrated subthreshold error rates for state preservation of a single logical qubit. In addition, the realization of universal quantum computation requires the implementation of logical entangling gates. Lattice surgery offers a practical approach for implementing such gates, particularly in planar quantum processor layouts. In this work, we demonstrate lattice surgery between two distance-three repetition-code qubits by splitting a single distance-three surface-code qubit. Using a quantum circuit fault-tolerant to bit-flip errors, we achieve an improvement in the value of the decoded $ZZ$ logical two-qubit observable compared to a similar non-encoded circuit. By preparing the surface-code qubit in initial states parametrized by a varying polar angle, we evaluate the performance of the lattice surgery operation for non-cardinal states on the logical Bloch sphere and employ logical two-qubit tomography to reconstruct the Pauli transfer matrix of the operation. In this way, we demonstrate the functional building blocks needed for lattice surgery operations on larger-distance codes based on superconducting circuits.

==> parts/literature_review.tex <==
%Quantum error correction is required to realize large-scale (practical) quantum computing \cite{Shor1996}.
%Topological error correction code, such as the surface code\cite{Kitaev2003, Dennis2002}, provide a straightforward strategy of constructing quantum error correction codes. The implementation of surface codes is based on the repeated measurement of syndrome operators, which can be carried out using auxiliary qubits \cite{Fowler2009, Raussendorf2007, Raussendorf2007a}. %The high error threshold of surface codes against circuit noise has 
%Thanks to its relatively high error threshold with respect to gate errors, the surface code has become an attractive target for experimental implementations on various platforms. The minimal surface code capable of repeatedly correcting single-qubit and two-qubit gate errors has been demonstrated on superconducting qubits \cite{Krinner2022, Acharya2023}, trapped ions\cite{Ryan-Anderson2021, Ryan-Anderson2024} and neutral atoms \cite{Bluvstein2022, Bluvstein2023}. 
%TODO: arb state prep.
%TODO: operations.
%A distn\cite{Andersen2020}
%These have been demonstrated on superconducting qubits\cite{Krinner2022, Acharya2023}

%A key capability of topological error correction codes is code deformation \cite{Bombin2006}: logical qubits can be encoded by a connected subset of a larger lattice. By changing which stabilizers are being measured over different rounds, one can fault-tolerantly re-encode the logical qubits and perform logical operations on them. 

%Lattice surgery \cite{Horsman2012} is a powerful tool for topological error correction codes where each logical qubit is a patches of active stabilizers, and the logical qubit operators are products of data qubit operators at the boundary of the patch. By measuring the correct parities between data qubits of different logical qubits, one can fault-tolerantly measure a two-logical-qubit operator. This is achieved by activating the stabilizers between the two patches, effectively merging them into a single patch, and subsequent deactivation of these stabilizers, splitting the large logical qubit into two smaller qubits.
%Lattice surgery-based logical operations stands out compared to transversal operations \cite{Gottesman1997} in that they are essentially code deformations, and only require the capability of repeated stabilizer measurements, and measurements and initialization of the data qubits in $X$ and $Z$ bases.

%trapped ions\cite{Ryan-Anderson2021, Ryan-Anderson2024},
\\

\textbf{Relevant Papers}
\begin{itemize}
    \item Lattice surgery can even be employed between logical qubits encoded in different sublattices of the same patch. Entanglement between a distance-4 3CX qubit and a Bacon-Shor qubit has recently been demonstrated on superconducting superconducting qubits with a heavy-hex connectivity \cite{Hetenyi2024}. (Ilya)
    \item Realization of building blocks of QEC on a neutral atom quantum 280-qubit quantum processor. Demonstrate distance scaling during transversal implementation of CNOT gate on $d=3,5,7$ surface codes. General limitation of all experiments: syndrome extraction rounds cannot be repeated, e.g. only single round of syndrome extraction during $d=7$ surface code state preparation makes protocol fault tolerant only up to $d=3$. Use correlations between extracted syndromes of both logical qubits to assemble hyperedge graph that is used for decoding, i.e. they use joint decoding graph for state preparation. Less relevant for this paper they also implement colour-code qubits, fault-tolerantly implement logical GHZ state and explore other QEC code. \cite{Bluvstein2023} (Michael)
    \item Lattice surgery operations can vary by the degree of independence of the individual qubits and strict adherence to the lattice geometry constraints. For systems with more flexible connectivity graphs, one can re-use the same auxiliary qubits in different roles, optimizing away certain operations. This has been demonstrated with trapped ions on the example of a distance-2 surface code teleportation and Bell state preparation experiment. (Experiment with 10 qubits, 8 data qubits, and 2 re-used ancilla qubits; use Y-based postselection similar to Ye2023, Bell state fidelity: 75\% with PS) \cite{Erhard2021} (Ilya).
    \item Ions, transversal CNOT on two Steane codes, 16 qubit in the QPU in total (quantum circuit not shown, but modularity went completely down the drain if there's just 2 aux qubits). Also demonstrate a fault-tolerant $H$-state preparation protocol ($\ket{H} = \frac{1}{\sqrt{2}}\ket{0} + \frac{e^{i\pi/4}}{\sqrt{2}}\ket{1}$) \cite{Postler2022} (Ilya)
    \item FT logical state teleportation using $d=3$ color code qubits in a system of 30 ion trap qubits. They also implement real-time error correction. Use one logical qubit $\ket{\psi}$ prepared in one of the cardinal states and FT preparation of logical Bell-pair to then FT measure $XX$ and $ZZ$ to teleport $\ket{\psi}$. They study adding QEC gadgets at different locations throughout the protocol. Justify using postselection for resource states (e.g. logical Bell pairs, or magic states) as they can be prepared in parallel to FT logic and used as needed. They prepare $\ket{\psi}$ by running an adaptive syndrome extraction sequence with up to three rounds followed by transversal Clifford operation. Perform FT readout of logical qubits again with adaptive syndrome extraction. Also find the QEC gadget to be the dominating error source in protocol. Experiment is realized on ion trap with the QCCD architecture meaning it is in principle modular and scalable.\cite{Ryan-Anderson2024} (Michael)
    \item Predecessor to \cite{Ryan-Anderson2024} where they operate a single $d=3$ color code qubit on 10-ion quantum device. Perform FT real-time error corrected state preparation of cardinal states as well as magic state preparation.  \cite{Ryan-Anderson2021} (Michael)
    \item Demonstrate distance scaling for $d=3,5$ surface codes on superconducting qubits being at the error threshold. Also perform distance scaling of a repetition code up to $d=25$. Observe limitation at around $10^{-6}$ caused by high-energy event. \cite{Acharya2023} (Michael)
    \item IBM Quantum Experience, [4,2,2] code, transversal set of gates (subset of Clifford group that can be implemented without too much pain in this encoding) \cite{Harper2019b} (Ilya)
    \item Repeated error correction on a distance-3 surface code \cite{Krinner2022} (Ilya)
    \item Magic state preparation on a $d=3$ surface code on superconducting qubits. Prepare center qubit of 3x3 data qubit lattice in state $\ket{\psi}$ and data qubits on the border in $\ket{0}$ or $\ket{+}$ depending on weight-2 stabilizer type. Show state preservation for cardinal states and other non-cardinal states. \cite{Ye2023a} (Michael)
    \item Arbitrary-phase rotations, non-fault-tolerant, Surface-7, Delft. \cite{Marques2021} (Ilya)
    \item FT preparation of a two qubit magic state within the four qubit error detecting code. Discussion of logical vs. physical state tomography and readout error mitigation. \cite{Gupta2024} --Log. Tomography like we do  (Lukas)
    \item FT operation of the Bacon-Shor code, comparing unitary initialization, Clifford gates and stabilizer measurement in nFT and FT variant.  \cite{Egan2021} --Similar "apples-to-apples comparison" in our case: raw and decoded ZZ parity to stress the significance of FT (Lukas)
    \item FT operation of the four qubit error detecting code for one log. qubit and nFT operation of the other.  \cite{Linke2017} -- Inserting artificial error and mapping out FT and nFT log. error rate, in our case one could do the same with an artificial Y error tracking ZZ and XX parity. (Lukas)
\end{itemize}
